Exponential separations between learning with and without quantum memory

We study the power of quantum memory for learning properties of quantum systems and dynamics, which is of great importance in physics and chemistry. Many state-of-the-art learning algorithms require access to an additional external quantum memory. While such a quantum memory is not required a priori, in many cases, algorithms that do not utilize quantum memory require much more data than those which do. We show that this trade-off is inherent in a wide range of learning problems. Our results include the following: (1) We show that to perform shadow tomography on an $n$-qubit state rho with $M$ observables, any algorithm without quantum memory requires $\Omega(\min(M, 2^n))$ samples of rho in the worst case. Up to logarithmic factors, this matches the upper bound of [HKP20] and completely resolves an open question in [Aar18, AR19]. (2) We establish exponential separations between algorithms with and without quantum memory for purity testing, distinguishing scrambling and depolarizing evolutions, as well as uncovering symmetry in physical dynamics. Our separations improve and generalize prior work of [ACQ21] by allowing for a broader class of algorithms without quantum memory. (3) We give the first tradeoff between quantum memory and sample complexity. We prove that to estimate absolute values of all $n$-qubit Pauli observables, algorithms with $k < n$ qubits of quantum memory require at least $\Omega(2^{(n-k)/3})$ samples, but there is an algorithm using $n$-qubit quantum memory which only requires $O(n)$ samples. The separations we show are sufficiently large and could already be evident, for instance, with tens of qubits. This provides a concrete path towards demonstrating real-world advantage for learning algorithms with quantum memory.

==> depolarize.tex <==
We are now prepared to establish the following result:
\begin{theorem}[Exponential hardness of fixed unitary task without a quantum memory]\label{thm:channelhard1}
Any learning algorithm without quantum memory requires
\begin{equation}
    T \geq \Omega\left( d^{1/4} \right),
\end{equation}
to correctly distinguish between the completely depolarizing channel $\mathcal{D}$ on $n$ qubits from a fixed, Haar-random unitary channel $\mathcal{U}[\rho] = U \rho U^\dagger$ on $n$ qubits with probability at least $2/3$.
% if the depth $T$ of the corresponding rooted tree $\mathcal{T}$ satisfies
% $T \leq \frac{\sqrt{d}}{4}$, then the probability of successfully distinguishing between $\mathcal{C} = \mathcal{D}$, the completely depolarizing channel on $n$ qubits, or $\mathcal{C} = \mathcal{U}$, a fixed, Haar-random unitary channel $\mathcal{U}[\rho] = U \rho U^\dagger$ on $n$ qubits, is upper bounded by
% \begin{equation}
% \mathcal{O}\!\left(\frac{T^2}{\sqrt{d}}\right)\,.
% \end{equation}
\end{theorem}

\noindent Hence, we established an exponential lower bound when the algorithm does not have a quantum memory. This is in stark contrast to learning algorithms with quantum memory. The following result from~\cite{aharonov2021quantum} states that a linear number of channel applications $T$ and quantum gates suffices.

\begin{theorem}[Fixed unitary task is easy with an $n$ qubit quantum memory~\cite{aharonov2021quantum}]
There exists a learning algorithm with $n$ qubits of quantum memory which, with constant probability, can distinguish $\mathcal{D}$ from a fixed, Haar-random $\mathcal{U}$ using only $T = \mathcal{O}(n)$ applications of the channel.  Moreover, the algorithm is gate efficient and has $\mathcal{O}(n)$ gate complexity.
\end{theorem}
\noindent The protocol is simply a swap test; the basic idea is that for a pure state $|\phi\rangle$ on $n$ qubits we have $\text{tr}(\mathcal{D}[|\phi\rangle \langle \phi|]^2) = \frac{1}{d}$ whereas $\text{tr}(\mathcal{U}[|\phi\rangle \langle \phi|]^2) = 1$.  The ability to obtain quantum interference between $\mathcal{D}[|\phi\rangle \langle \phi|]$ and a copy of itself $\mathcal{D}[|\phi\rangle \langle \phi|]$ (or $\mathcal{U}[|\phi\rangle \langle \phi|]$ and a copy of itself $\mathcal{U}[|\phi\rangle \langle \phi|]$) is enabled by the $n$ qubit quantum memory which can store a single copy of the state.

We now turn to a proof of Theorem~\ref{thm:channelhard1}, which is our main result about the fixed unitary problem.  We note that a special case of this theorem was proved in~\cite{aharonov2021quantum}, namely where the learning protocol (see Definition~\ref{def:treechannel}) does not have an auxiliary system, i.e.~$\mathcal{H}_{\text{aux}}$ is a trivial Hilbert space.  The inclusion of an $\mathcal{H}_{\text{aux}}$ of arbitrary size $d' = 2^{n'}$ is our main technical contribution here; our proof will follow the same contours as that of~\cite{aharonov2021quantum}, but with substantive modifications and generalizations. The original proof .


\begin{proof}
The proof begins by utilizing Lemma~\ref{lem:lecam-channel}, which gives
\begin{equation}
    \frac{2}{3} \leq \frac{1}{2} \sum_{\ell \in \mathrm{leaf}(\mathcal{T})} \left| p^{\mathcal{D}}(\ell) - \left( \Expect_{\mathcal{U}} p^{\mathcal{U}}(\ell) \right) \right|.
\end{equation}
The goal now would be to obtain an upper bound right hand side.
It is convenient to establish some notation.  Each root-to-leaf path in $\mathcal{T}$ is specified by a sequence of vertices $v_0, v_1,..., v_T$ where $v_0 = r$ is the root and $v_T = \ell$ is a leaf.  Moreover, the leaf $\ell$ determines the entire root-to-leaf path: it is the shortest path from that leaf to the root.  So knowing $\ell$ is the same as knowing the entire path $v_0 = r, v_1,...,v_{T-1}, v_T = \ell$. 
Recall from Eq.~\eqref{eq:prob-channel-node} and following the root-to-leaf path $v_0 = r, v_1,...,v_{T-1}, v_T = \ell$, the probability of the leaf $\ell$ under the channel $\mathcal{C}$ is
\begin{equation}
    p^{\mathcal{C}}(\ell) = \prod_{t=1}^T \left(w_{v_t} d d' \, \langle \psi_{v_t}|\,(\mathcal{C} \otimes \mathcal{I}_{\text{\rm aux}})[|\phi_{v_{t-1}}\rangle \langle \phi_{v_{t-1}}|] \,|\psi_{v_t}\rangle \right),
\end{equation}
where each $\ket{\phi_{v_{t-1}}}, \ket{\psi_{v_{t-1}}}$ lives in $(d d')$-dimensional Hilbert space $\mathcal{H} \simeq \mathcal{H}_{\text{\rm main}} \otimes \mathcal{H}_{\text{\rm aux}}$ from Definition~\ref{def:treechannel}.
To analyze the probability, we let
\begin{align}
\label{E:Phibig1}
|\Phi_\ell\rangle &= |\phi_{v_0}\rangle  \otimes |\phi_{v_1}\rangle \otimes \cdots \otimes |\phi_{v_{T-1}}\rangle \\
\label{E:Psibig1}
|\Psi_\ell\rangle &= |\psi_{v_1}\rangle  \otimes |\psi_{v_2}\rangle \otimes \cdots \otimes |\psi_{v_T}\rangle  \\
\label{E:Wbig1}
W_\ell &= w_{v_1} w_{v_2} \cdots w_{v_T}
\end{align}
where $v_0 = r$ and $v_T = \ell$.  Notice that $|\Phi_\ell\rangle$ and $|\Psi_\ell\rangle$ each live in $\mathcal{H}^{\otimes T}$.
Recall from Definition~\ref{def:treechannel}, for any node $u$, the set $\{\sqrt{w_v d d'}\,|\psi_v\rangle \langle \psi_v|\}_{v \in \mathrm{child}(u)}$ is a POVM.
Hence, we have $\sum_{v \in \mathrm{child}(u)} w_v d d' \,|\psi_v\rangle \langle \psi_v| = \mathds{1}_{\text{main}} \otimes \mathds{1}_{\text{aux}}$.
It is not hard to use this fact to derive the following identity
\begin{align}
\label{E:Widentity1}
\sum_{\ell \,\in\, \text{leaf}(\mathcal{T})} (d d')^T W_\ell \, |\Psi_\ell\rangle \langle \Psi_\ell| &= (\mathds{1}_{\text{main}} \otimes \mathds{1}_{\text{aux}})^{\otimes T}
\end{align}
and so accordingly $\sum_{\ell \,\in\, \text{leaf}(\mathcal{T})} W_\ell = 1$.

With these notations at hand, we can write $p^{\mathcal{D}}(\ell)$ diagrammatically as
\begin{align}
\label{E:PS1}
    \includegraphics[scale=.32, valign = c]{PS1.png}.
\end{align}
For $\mathbb{E}_{\text{\rm Haar}}[p^{\mathcal{U}}(\ell)]$, we utilize the Haar averaging of unitary group discussed in Section~\ref{sec:haaraverageUd} to obtain
\begin{align}
\label{E:QS1}
    \includegraphics[scale=.32, valign = c]{QS1.png}
\end{align}
where the solid lines correspond to $\mathcal{H}_{\text{main}}^{\otimes T}$ and the dotted lines correspond to $\mathcal{H}_{\text{aux}}^{\otimes T}$\,.  It is convenient to let $p_{\sigma, \tau}(\ell)$ denote the summand of~\eqref{E:QS1}.
We now use the triangle inequality in combination with the Cauchy-Schwarz inequality to write
\begin{align}
\label{E:firstineq1}
&\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)]| \nonumber \\
&\qquad \leq \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathds{1},\mathds{1}}(\ell)| + \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\sigma \not = \mathds{1}}|p_{\sigma, \mathds{1}}(\ell)| +  \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\tau \not = \mathds{1}, \,\sigma}|p_{\sigma, \tau}(\ell)| \,.
\end{align}
We will bound each term in turn.

\subsubsection*{First term}
Applying Cauchy-Schwarz to the first term in~\eqref{E:firstineq1} we find that it is less than or equal to
\begin{align}
\label{E:11bound}
    \includegraphics[scale=.32, valign = c]{11bound.png}
\end{align}
We can remove the absolute values on the diagrammatic term since it is strictly positive; this enables us to perform the sum over leaves $\sum_{\ell \in \mathrm{leaf}(\mathcal{T})}$ and via the identity given in~\eqref{E:Widentity1}. The first term in~\eqref{E:firstineq1} can now be written as
\begin{equation}
\label{E:Wg1remain1}
\frac{d^T}{2}\,\left|\text{Wg}^U(\mathds{1},d) - \frac{1}{d^T}\right|\,.
\end{equation}
Since by Corollary~\ref{cor:WgU1bd} we have $|\text{Wg}^U(\mathds{1},d) - \frac{1}{d^T}| \leq \mathcal{O}(T^{7/2}/d^{T+2})$ for $T < \left(\frac{d}{\sqrt{6}}\right)^{4/7}$, Eqn.~\eqref{E:Wg1remain1} is $\mathcal{O}(T^{7/2}/d^{2})$ and so
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathds{1},\mathds{1}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^{7/2}}{d^2}\right)\,.
\end{equation}

\subsubsection*{Second term}
Next we treat the second term in~\eqref{E:firstineq1}, namely $\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\sigma \not = \mathds{1}}|p_{\sigma, \mathds{1}}(\ell)|$.  Utilizing the Cauchy-Schwarz inequality, this term is less than or equal to
\begin{align}
\label{E:cs2ndterm}
    \includegraphics[scale=.32, valign = c]{cs2ndterm.png}
\end{align}
We can dissect the middle term in the summand using the H\"{o}lder inequality
\begin{align}
    \includegraphics[scale=.32, valign = c]{Holder1.png}
\end{align}
and notice that $\|\sigma\|_\infty = 1$.  Furthermore, using the fact that the matrix inside the 1-norm on the right-hand side is positive semi-definite, we can replace the 1-norm with the trace and find the bound
\begin{align}
    \includegraphics[scale=.32, valign = c]{1normproperty1.png}
\end{align}
Thus~\eqref{E:cs2ndterm} is upper bounded by
\begin{align}
    \includegraphics[scale=.32, valign = c]{postinfnorm1.png}
\end{align}
Then applying the identity~\eqref{E:Widentity1} we are left with
\begin{equation}
\frac{d^T}{2} \sum_{\sigma \not = \mathds{1}} |\text{Wg}^U(\sigma^{-1},d)|
\end{equation}
which is less than or equal to $\mathcal{O}(T^2/d)$ by Lemma 6 of~\cite{aharonov2021quantum}.  In summary, we have
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\sigma \not = \mathds{1}}|p_{\sigma, \mathds{1}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^2}{d}\right)\,.
\end{equation}

\subsubsection*{Third term}
Finally we treat the third term in~\eqref{E:firstineq1}, namely $\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\tau \not = \mathds{1}, \,\sigma}|p_{\sigma, \tau}(\ell)|$, which is the most difficult case.  Leveraging the Cauchy-Schwarz inequality, this term is upper bounded by
\begin{align}
\label{E:thirdterm1}
    \includegraphics[scale=.32, valign = c]{thirdterm1.png}
\end{align}
Applying the H\"{o}lder inequality to the second term in the summand as before, we find
\begin{align}
\label{E:Holder2}
    \includegraphics[scale=.32, valign = c]{Holder2.png}
\end{align}
where $\|\sigma\|_\infty = 1$.  We also use the convenient inequality
\begin{align}
\label{E:thirdterm1}
\includegraphics[scale=.32, valign = c]{tensorreorder1.png}
\end{align}
to reorganize the order of the tensor legs; we have used the H\"{o}lder inequality to go from the middle term to the last term, and the fact that $\|\tau\|_\infty = 1$.

For a fixed permutation $\tau^{-1}$, we can decompose it into cycles $C_1 C_2 \cdots C_{\#(\tau^{-1})}$.  We say that $i \to j$ is in the $m$th cycle $C_m$ if $C_m = (\cdots ij \cdots)$.  Using this notation, for fixed $\tau^{-1} = C_1 C_2 \cdots C_{\#(\tau^{-1})}$ and letting $v_0 = r, v_1,...,v_{T-1}, v_T = \ell$ be the root-to-leaf path terminating in $\ell$, we have

\begin{lemma}
    We have the following identity represented using tensor network diagrams.
    \begin{align}
    \label{E:cycledecomp1}
        \includegraphics[scale=.32, valign = c]{cycledecomp1.png}
    \end{align}
\end{lemma}

\begin{proof}
    Take any cycle $C_m$ and any $i\to j\in C_m$. The solid leg of $\bra{\phi_{v_{i - 1}}}$ is dangling and the dotted leg connects to $\bra{\psi_{v_i}}$. Similarly, the solid leg of $\ket{\phi_{v_{j-1}}}$ is dangling and the dotted leg connects to $\ket{\psi_{v_j}}$. Lastly, the solid leg of $\bra{\psi_{v_i}}$ connects to $\ket{\psi_{v_j}}$. This accounts for all legs among $\phi_{v_{i-1}}$, $\psi_{v_i}$, $\phi_{v_{j - 1}}$, and $\psi_{v_j}$, so the part of the diagram on the left of \eqref{E:cycledecomp1} that corresponds to these four states is not connected to the rest of the diagram. In this fashion, we conclude that the diagram on the left is a tensor product of the diagrams on the left for all $m$ and $i\to j\in C_m$, from which the lemma follows. We refer to Figure~\ref{fig:example_cycledecomp} for an illustration. \TODO{}
    \begin{figure}[h]\label{fig:example_cycledecomp}
        \caption{\color{red} {[example illustration of the decomposition for alphabet size 2 or 3, TODO]}}
    \end{figure}
\end{proof}

We would like to convert the product of trace norms in \eqref{E:cycledecomp1} into a product of traces. We do so via the following basic estimate. First, for any $i\in[T]$, define the unnormalized density operator $\widetilde{\rho}_{v_i} \in \text{Mat}_{d \times d}(\mathbb{C})$ by
\begin{align}
\label{E:rhotildedef}
    \includegraphics[scale=.32, valign = c]{rhotildedef.png}
\end{align}

\begin{lemma}
    For any $i\to j\in C_m$, the corresponding term on the right-hand side of \eqref{E:cycledecomp1} is upper bounded by $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})$. In particular, \eqref{E:cycledecomp1} is at most \begin{equation}\label{E:productwithsqrt1}
        \prod^{\#(\tau^{-1})}_{m = 1}\prod_{i\to j\in C_m} \sqrt{\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})}.
    \end{equation}
\end{lemma}

\begin{proof}
Using the relations $\|A\|_1 = \|A\otimes A^\dagger\|_1^{1/2} \leq \|\text{SWAP}  \cdot (A\otimes A^\dagger)\|_1^{1/2}$, we find
\begin{align}
% \label{E:SWAPineq1}
    \includegraphics[scale=.32, valign = c]{SWAPineq1.png} \nonumber
\end{align}
Since the operator inside the 1-norm on the right-hand side is clearly positive semi-definite, we can replace the 1-norm with a trace, namely
\begin{align}
\label{E:1normproperty2}
    % \includegraphics[scale=.32, valign = c]{1normproperty2.png}
    \includegraphics[scale=.32, valign = c]{figs/trprod_color.png}
\end{align}
Observe that we can equivalently rewrite~\eqref{E:1normproperty2} as $\sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})}$\,, where $\wt{\rho}_{v_i}$ is the component of the diagram denoted in red and $\wt{\rho}_{v_j}$ is the one in blue, yielding the first part of the lemma. The second follows from plugging this into the right-hand side of Eqn.~\eqref{E:cycledecomp1}.
\end{proof} 

To bound \eqref{E:productwithsqrt1}, it is convenient to develop some notation for cycles $C_m$\,.  The usual notation for a cycle of length $p$ (which for us is less than or equal to $T$) is $C_m = (a_1 a_2 \cdots a_p)$ where in our setting $\{a_1, a_2,...,a_p\} \subseteq \{1,2,...,T\}$.  We will decorate each $a_i$ by an additional subscript as $a_{m,i}$ to remember that it that belongs to the $m$th cycle $C_m$. Similarly, we will sometimes write $p = |C_m|$ to remind ourselves that it depends on $m$.  In this notation, we can write \eqref{E:productwithsqrt1} as a product of
\begin{equation}
\label{E:cycletobound1}
% \prod_{i \to j \, \in C_m} \sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})}\ = 
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}} \widetilde{\rho}_{v_{a_{m,2}}})}  \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,2}}} \widetilde{\rho}_{v_{a_{m,3}}})} \,\cdots \, \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p-1}}} \widetilde{\rho}_{v_{a_{m,p}}})} \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})}
\end{equation}
over the different $m = 1, \ldots, \#(\tau^{-1})$.
We can further process the above expression for a given $m$.
We proceed by analyzing two cases: (i) $p = |C_m|$ is even, and (ii) $p = |C_m|$ is odd. \\ \\
\textbf{Case 1:} \textit{$p$ is even.} Each term in Eqn.~\eqref{E:cycletobound1} has the form $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}$ except for the last term; however, if we treat the $i$ subscripts of $a_{m,i}$ modulo $p$, then we can write the last term as $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,p+1}}})}$\,.  We elect to use this notation.  Then we can rearrange and group the terms in Eqn.~\eqref{E:cycletobound1} as follows
\begin{equation}
\left(\prod_{i\text{ odd}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, the above is upper bounded by
\begin{equation}
\frac{1}{2} \prod_{i\text{ odd}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})\,.
\end{equation}
We will call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. \\ \\
\textbf{Case 2:} \textit{$p$ is odd.} Again consider the product in Eqn.~\eqref{E:cycletobound1}.  We can rearrange and group terms as
\begin{equation}
\label{E:oddsplit1}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})}\left(\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
If two matrices $A,B$ are Hermitian and positive semi-definite, then using Cauchy-Schwarz combined with operator norm inequalities we have $\text{tr}(AB) \leq \|A\|_2 \, \|B\|_2 \leq \|A\|_1 \, \|B\|_1 \leq \text{tr}(A) \, \text{tr}(B)$.  Accordingly, we have $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})} \leq \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}}) \, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}$ and so~\eqref{E:oddsplit1} is upper bounded by
\begin{equation}
\left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})} \prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Again using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, we have the upper bound
\begin{equation}
\frac{1}{2} \,\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})
\end{equation}
where we analogously call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. 

In both cases, note that $R_{m,\,-}$ and $R_{m,\,+}$ implicitly depend on the leaf $\ell$, so we will denote them by $R^{\ell}_{m,\,-}$ and $R^{\ell}_{m,\,+}$ when we wish to make this dependence explicit.\\ \\
\indent Putting together our notation and bounds from Case 1 and Case 2, we find that Eqn.~\eqref{E:productwithsqrt1} is upper bounded by
\begin{align}
\label{E:multipleTs}
\prod_{m=1}^{\#(\tau^{-1})} \,\prod_{i \to j \, \in C_m} \sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})} &\leq \frac{1}{2^{\#(\tau^{-1})}} \prod_{m=1}^{\#(\tau^{-1})} \left(R_{m,-} + R_{m,+} \right) \nonumber \\
&= \frac{1}{2^{\#(\tau^{-1})}} \sum_{i_1,...,i_{\#(\tau^{-1})} = \pm} R_{1,i_1} R_{2,i_2} \cdots R_{\#(\tau^{-1}), i_{\#(\tau^{-1})}}\,.
\end{align}
Each term in the sum in the last line of~\eqref{E:multipleTs} is a product of terms like $\text{tr}(\widetilde{\rho}_{v_i})$ and $\text{tr}(\widetilde{\rho}_{v_j} \widetilde{\rho}_{v_k})$.  But the key point is that we have arranged the equations so that each term in the sum has $\widetilde{\rho}_{v_i}$ for each $i = 1,...,T$ appear \textit{exactly once}.  This has the following highly useful consequence.


\begin{lemma}\label{lem:collapse}
    Fix any $i_1,...,i_{\#(\tau^{-1})} \in \{+,-\}$. Then
    \begin{equation}
        \label{E:sboundhard1}
        \sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} (d d')^T \,W_\ell \, R^{\ell}_{1,i_1} R^{\ell}_{2,i_2} \cdots R^{\ell}_{\#(\tau^{-1}), i_{\#(\tau^{-1})}} \le d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2}\right\rfloor}
    \end{equation}
where $L(\tau^{-1})$ is the length of the longest cycle in $\tau^{-1}$.
\end{lemma}

\begin{proof}
    For ease of notation, we will let $R^{\ell}_j\triangleq R^{\ell}_{j,i_j}$.
    Recall from~\eqref{E:Wbig1} that $W_\ell = w_{v_1} w_{v_2} \cdots w_{v_T}$ and note that
    \begin{equation}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \widetilde{\rho}_{v} = \langle \phi_{\text{parent}(v)} | \phi_{\text{parent}(v)}\rangle\, \mathds{1}_{d \times d} = \mathds{1}_{d \times d}\,.
    \end{equation}
    Accordingly we have that for any $\rho\in\text{Mat}_{d\times d}(\mathbb{C})$,
    \begin{align}
        \label{E:2tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\, w_{v} \, \text{tr}(\widetilde{\rho}_{v} \, \rho ) = \text{tr}(\rho)\,,
    \end{align}
    and in particular, for $\rho = \mathds{1}$,
    \begin{align}
        \label{E:1tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \text{tr}(\widetilde{\rho}_{v}) &= d.
    \end{align}
    We now turn to bounding the left-hand side of \eqref{E:sboundhard1}. Recalling that $\prod_j R^{\ell}_j$ as a product of terms like $\Tr(\wt{\rho}_{v_i})$ and $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_i'})$, we will define some sets of indices encoding this data. Let $S^{(T)}_1\subseteq[T]$ denote the indices $i$ for which $\Tr(\wt{\rho}_{v_i})$ appears in $\prod_j R^{\ell}_j$, and let $S^{(T)}_2\subseteq[T]\times[T]$ denote the set of (unordered) pairs $(i,i')$ for which $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})$ appears, so that for any root-to-leaf path in $\calT$ consisting of nodes $v_1,\ldots,v_T = \ell$, we have
    \begin{equation}
        \label{eq:prodRs}
        \prod_j R^{\ell}_j = \prod_{i\in S^{(T)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i')\in S^{(T)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})
    \end{equation} by definition. Now construct $S^{(t)}_1\subseteq[t]$ and $S^{(t)}_2\subseteq[t]\times[t]$ for $1 \le t < T$ inductively as follows. If $t\in S^{(t)}_1$ then define $S^{(t-1)}_1 \triangleq S^{(t)}_1 \backslash \brc{t}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2$. Otherwise if $(t,t')\in S^{(t)}_2$ for some $t' < t$, then define $S^{(t-1)}_1 \triangleq S^{(t-1)}_1 \cup \brc{t'}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2 \backslash \brc{(t,t')}$. We collect some basic observations about these two set sequences:
    
    \begin{observation}\label{obs:singleton}
        For every $i\in S^{(T)}_1$, we have that $i\in S^{(i)}_1$.
    \end{observation}
    
    \begin{observation}\label{obs:pair}
        For every $(i,i')\in S^{(T)}_2$, if $i\le i'$ then $i\in S^{(i)}_1$ while $i'\not\in S^{(i')}_1$.
    \end{observation}
    
    The reason for defining these set sequences is that we can extract $\wt{\rho}_{v_T}$ from the product on the right-hand side of \eqref{eq:prodRs} and apply \eqref{E:1tracebound1} (resp. \eqref{E:2tracebound1}) if $T\in S^{(T)}_1$ (resp. $(T,t')\in S^{(T)}_2$ for some $t' < T$) to obtain \begin{equation}
        \label{eq:induct_prodRs}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j = d^{\bone{T\in S^{(T)}_1}}\sum_{u: \,\text{depth}(u) = T - 1} (dd')^{T-1} W_u \prod_{i\in S^{(T-1)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i') \in S^{(T-1)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}}),
    \end{equation} where $W_u = w_{v_1}\cdots w_{v_{T-1}}$ if the path from root to $u$ in $\calT$ consists of $v_1,\ldots,v_{T-1} = u$.
    Proceeding inductively, we can express the right-hand side of \eqref{eq:induct_prodRs} as \begin{equation}
        d^{\sum^T_{t=1} \bone{t\in S^{(t)}_1}}.
    \end{equation} By Observations~\ref{obs:singleton} and \ref{obs:pair}, $\sum^T_{t=1}\bone{t\in S^{(t)}_1} = |S^{(T)}_1| + |S^{(T)}_2|$. Because every even cycle $C_m$ of $\tau^{-1}$ contributes $|C_m|/2$ pairs to $S^{(T)}_2$, and every odd cycle $C_m$ contributes $\floor{|C_m|/2}$ pairs to $S^{(T)}_2$ and one element to $S^{(T)}_1$, we conclude that
    \begin{align}
        \label{E:sboundhard2}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j &= d^{\sum_{m=1}^{\#(\tau^{-1})} \left\lceil \frac{|C_m|}{2} \right\rceil} \nonumber \\
        &= d^{\frac{T}{2} - \sum_{m=1}^{\#(\tau^{-1})} \left\lfloor \frac{|C_m|}{2} \right\rfloor} \nonumber \\
        &\leq d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2} \right\rfloor}
    \end{align}
    as claimed.
\end{proof}

Putting all of our previous analysis together, in particular by combining Eq.~\eqref{E:Holder2}, \eqref{E:thirdterm1}, \eqref{E:cycledecomp1}, \eqref{E:productwithsqrt1}, \eqref{E:multipleTs}, and \eqref{E:sboundhard1}, we arrive at
\begin{equation}
\sum_{\ell \, \in \, \text{leaf}(\mathcal{T})} \sum_{\tau \not = \mathds{1}, \,\sigma}|p_{\sigma, \tau}(s)| \leq d^{T} \sum_{\sigma} |\text{Wg}^U(\sigma^{-1}, d)| \sum_{\tau \not = \mathds{1}} d^{- \left\lfloor \frac{L(\tau^{-1})}{2} \right\rfloor} \,.
\end{equation}
The first sum on the right-hand side is bounded by $d^T \sum_{\sigma} |\text{Wg}^U(\sigma^{-1}, d)| \leq 1 + \mathcal{O}\!\left( \frac{T^2}{d}\right)$.  Considering the second sum on the right-hand side, let $N(T,\ell)$ be the number of permutations in $S_T$ where the length of the longest cycle is $\ell$.  Then the second sum can be written as
\begin{equation}
\label{E:sumNTell}
\sum_{\ell = 2}^T N(T,\ell) \, d^{- \left\lfloor \frac{\ell}{2} \right\rfloor}
\end{equation}
where we omit $k = 1$ from the sum since it corresponds to the identity permutation.  Since $N(T,\ell) \leq \binom{T}{\ell} \, \ell! = \frac{T!}{(T - \ell)!} < T^\ell$,~\eqref{E:sumNTell} is upper bounded by
\begin{equation}
\sum_{\ell = 2}^\infty T^\ell  \, d^{- \left\lfloor \frac{\ell}{2} \right\rfloor} = \frac{(1 + T) \frac{T^2}{d}}{1 - \frac{T^2}{d}} = \frac{T^3}{d} + \frac{T^2}{d} + \mathcal{O}\!\left(\frac{T^5}{d^2}\right)\,.
\end{equation}
%we observe that the number of permutations of $T$ items with $L$ disjoint cycles (including counting cycles of unit length) is given by the unsigned Stirling numbers of the first kind ${ T\brack L}$.  As such we can write
%\begin{equation}
%\label{E:1stirling1}
%\sum_{\tau \not = \mathds{1}} d^{\#(\tau^{-1})/2}  = \sum_{L=0}^{T-1} { T\brack L}  d^{L/2} 
%\end{equation}
%where we only sum up to $T-1$ since $L = T$ corresponds to $\tau^{-1} = \mathds{1}$ which is omitted from the sum.  Unsigned Stirling numbers of the first kind enjoy the identity $\sum_{L=0}^T { T\brack L} \, x^L = x (x+1) \cdots (x + T - 1)$ and so~\eqref{E:1stirling1} is equivalent to
%\begin{align}
%d^{1/2} \left(d^{1/2}  + 1\right) \cdots \left(d^{1/2}  + T-1 \right) - d^{T/2} &\le d^{T/2}\left(\exp\left(\frac{T(T-1)}{d^{1/2}}\right) - 1\right).
%\end{align}
Now if $T \le o(d^{1/3})$, then this quantity is $o(1)$ for some absolute constant $c > 0$. Altogether, we find
\begin{equation}
\frac{1}{2}\sum_{\ell\,\in\,\text{leaf}(\mathcal{T})} \sum_{\tau \not = \mathds{1}, \,\sigma}|p_{\sigma, \tau}(\ell)| \leq o\!\left(1\right)\,.
\end{equation}
% \\ \\
% \indent In totality, for $T \leq \frac{\sqrt{d}}{4}$ we find
% \begin{equation}
% \frac{1}{2}\sum_s |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)]| \leq o\!\left(1\right)
% \end{equation}
% which is the claimed result.

\end{proof}

\textcolor{red}{[Discuss corollary involving states; here the auxiliary system is extraneous and so can set it to be trivial; reduce to the corollary already presented in~\cite{aharonov2021quantum}]}

\subsection{Symmetry distinction problem}

\textcolor{red}{[In progress]}

\begin{proof}

The probability distribution $p^{\mathcal{D}}(\ell)$ is notated the same way as before.
We can depict $\mathbb{E}_{\text{\rm Haar}}[p^{\mathcal{O}}(\ell)]$ diagrammatically by
\begin{align}
\label{E:OQS1}
    \includegraphics[scale=.32, valign = c]{OQS1.pdf}
\end{align}
where $p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{O}}(\ell)$ denotes the summand.  Similarly $\mathbb{E}_{\text{\rm Haar}}[p^{\mathcal{S}}(\ell)]$ is given by
\begin{align}
\label{E:SpQS1}
    \includegraphics[scale=.32, valign = c]{SpQS1.pdf}
\end{align}
where here $p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{S}}(\ell)$ denotes the summand.  As before, we use the triangle inequality in combination with the Cauchy-Schwarz inequality to write the two inequalities
\begin{align}
\label{E:Ofirstineq1}
&\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{O}}(\ell)]| \nonumber \\
&\qquad \leq \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathfrak{e}, \mathfrak{e}}^{\mathcal{O}}(\ell)| + \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathfrak{e}}|p_{\mathfrak{m}, \mathfrak{e}}^{\mathcal{O}}(\ell)| +  \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathfrak{e}, \,\mathfrak{n}}|p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{O}}(\ell)| \,.
\end{align}
and
\begin{align}
\label{E:Spfirstineq1}
&\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{S}}(\ell)]| \nonumber \\
&\qquad \leq \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathfrak{e}, \mathfrak{e}}^{\mathcal{S}}(\ell)| + \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathfrak{e}}|p_{\mathfrak{m}, \mathfrak{e}}^{\mathcal{S}}(\ell)| +  \frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathfrak{e}, \,\mathfrak{n}}|p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{S}}(\ell)| \,.
\end{align}
We will bound the right-hand sides of~\eqref{E:Ofirstineq1} and~\eqref{E:Spfirstineq1} term by term.


\subsubsection*{First term for $O(d)$ case}
We apply the Cauchy-Schwarz inequality to the first term in~\eqref{E:Ofirstineq1} to find the upper bound
\begin{align}
\label{E:O11bound}
    \includegraphics[scale=.32, valign = c]{O11bound.pdf}
\end{align}
As in the unitary setting, we remove the absolute values on the diagrammatic term by virtue of its positivity, and sum over leaves to get
\begin{equation}
\label{E:OWg1remain1}
\frac{d^T}{2}\,\left|\text{Wg}^O(\sigma_{\mathfrak{e}},d) - \frac{1}{d^T}\right|\,.
\end{equation}
Using Corollary~\ref{cor:WgO1bd} which gives us $|\text{Wg}^O(\sigma_{\mathfrak{e}},d) - \frac{1}{d^T}| \leq \mathcal{O}(T^{7}/d^{T+2})$ for $T < \left(\frac{d}{12}\right)^{2/7}$, we immediately find
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathfrak{e}, \mathfrak{e}}^{\mathcal{O}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^{7}}{d^2}\right)\,.
\end{equation}

\subsubsection*{First term for \normalfont $\text{Sp}(d/2)$ \normalfont \textbf{case}}

We recapitulate the same manipulations in the symplectic case.  Applying the Cauchy-Schwarz inequality to the first term in~\eqref{E:Spfirstineq1} gives us the upper bound
\begin{align}
\label{E:Sp11bound}
    \includegraphics[scale=.32, valign = c]{Sp11bound.pdf}
\end{align}
We again remove the absolute values around the diagrammatic term, and sum over leaves to find
\begin{equation}
\label{E:SpWg1remain1}
\frac{d^T}{2}\,\left|\text{Wg}^{\text{Sp}}(\sigma_{\mathfrak{e}},d/2) - \frac{1}{d^T}\right|\,.
\end{equation}
Using the analogous Corollary~\ref{cor:WgSp1bd} which provides the bound $|\text{Wg}^O(\sigma_{\mathfrak{e}},d) - \frac{1}{d^T}| \leq \mathcal{O}(T^{7/2}/d^{T+2})$ for $T < \left(\frac{d}{6}\right)^{2/7}$, we have
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - p_{\mathfrak{e}, \mathfrak{e}}^{\mathcal{S}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^{7/2}}{d^2}\right)\,.
\end{equation}


\subsubsection*{Second term for $O(d)$ case}
Applying Cauchy-Schwarz to the second term in~\eqref{E:Ofirstineq1}, we find the upper bound
\begin{align}
\label{E:Ocs2ndterm}
    \includegraphics[scale=.32, valign = c]{Ocs2ndterm.pdf}
\end{align}
The diagrammatic term can be bounded using the H\"{o}lder inequality
\begin{align}
    \includegraphics[scale=.32, valign = c]{OHolder1.pdf}
\end{align}
which we can further simplify since $\|\Delta_{\mathfrak{m}}\|_\infty = 1$.  The diagrammatic term inside the 1-norm is positive semi-definite, and so its one norm is simply its trace, i.e.~
\begin{align}
\label{E:1normistrace1}
    \includegraphics[scale=.32, valign = c]{1normproperty1.png}
\end{align}
Then~\eqref{E:Ocs2ndterm} has the upper bound
\begin{align}
    \includegraphics[scale=.32, valign = c]{O1postinfnorm1.pdf}
\end{align}
Summing over leaves we arrive at
\begin{equation}
\frac{d^T}{2} \sum_{\mathfrak{m} \not = \mathfrak{e}} |\text{Wg}^{O}(\sigma_{\mathfrak{m}}^{-1},d)|
\end{equation}
which is upper bounded by $\mathcal{O}(T^7/d^2) + \mathcal{O}(T^2/d)$ using Corollary~\ref{cor:WgO1bd} in combination with Lemma 8 of~\cite{aharonov2021quantum}.  The ultimate result is
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathds{1}}|p_{\mathfrak{m}, \mathfrak{e}}^{\mathcal{O}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^7}{d^2}\right) + \mathcal{O}\!\left(\frac{T^2}{d}\right)\,.
\end{equation}

\subsubsection*{Second term for \normalfont $\text{Sp}(d/2)$ \normalfont \textbf{case}}

A similar proof holds in the symplectic setting. We likewise apply Cauchy-Schwarz to the second term in~\eqref{E:Spfirstineq1} to obtain the upper bound
\begin{align}
\label{E:Spcs2ndterm}
    \includegraphics[scale=.32, valign = c]{Spcs2ndterm.pdf}
\end{align}
Next we use the H\"{o}lder inequality, along with the operator inequality $\|AB\|_\infty \leq \|A\|_\infty \|B\|_\infty$, to obtain
\begin{align}
    \includegraphics[scale=.32, valign = c]{SpHolder1.pdf}
\end{align}
Here we also have $\|\textbf{J}^t\|_\infty = \|\Delta_{\mathfrak{m}}' \|_\infty = 1$.  As before, the diagrammatic term inside the 1-norm is positive semi-definite and so we can use~\eqref{E:1normistrace1}.  Thus we arrive at an upper bound for~\eqref{E:Spcs2ndterm}, namely
\begin{align}
    \includegraphics[scale=.32, valign = c]{Sp1postinfnorm1.pdf}
\end{align}
As before we sum over leaves, giving us
\begin{equation}
\frac{d^T}{2} \sum_{\mathfrak{m} \not = \mathfrak{e}} |\text{Wg}^{\text{Sp}}(\sigma_{\mathfrak{m}}^{-1},d/2)|\,.
\end{equation}
This is is upper bounded by $\mathcal{O}(T^{7/2}/d^2) + \mathcal{O}(T^2/d)$ using Corollary~\ref{cor:WgSp1bd} in combination with Lemma 10 of~\cite{aharonov2021quantum}, and so in the end we obtain
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{m} \not = \mathds{1}}|p_{\mathfrak{m}, \mathfrak{e}}^{\mathcal{S}}(\ell)| \leq \mathcal{O}\!\left(\frac{T^{7/2}}{d^2}\right) + \mathcal{O}\!\left(\frac{T^2}{d}\right)\,.
\end{equation}


\subsubsection*{Third term for $O(d)$ case}
The third term in~\eqref{E:Ofirstineq1} is $\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{n} \not = \mathfrak{e}, \,\mathfrak{m}}|p_{\mathfrak{m},\mathfrak{n}}^{\mathcal{O}}(\ell)|$.  Applying the Cauchy-Schwarz inequality we obtain the upper bound
\begin{align}
\label{E:Othirdterm1}
    \includegraphics[scale=.32, valign = c]{Othirdterm1.pdf}
\end{align}
Similar to above, we can upper bound the diagrammatic term using the H\"{o}lder inequality as
\begin{align}
\label{E:OHolder2}
    \includegraphics[scale=.32, valign = c]{OHolder2.pdf}
\end{align}
with $\|\Delta_{\mathfrak{m}}\|_\infty = 1$.  Letting $\lambda_{\mathfrak{n}}$ and $\rho_{\mathfrak{n}}$ be permutations on $S_{T}$ that we will specify shortly, we can again use the H\"{o}lder inequality to obtain
\begin{align}
\includegraphics[scale=.32, valign = c]{Otensorreorder1.pdf}
\end{align}
where we have used $\|\lambda_{\mathfrak{n}}^{-1}\|_\infty = \|\rho_{\mathfrak{n}}\|_\infty = 1$.  Now we turn to constructing a $\lambda_{\mathfrak{n}}$ and $\rho_{\mathfrak{n}}$ that will be convenient for us in the next stage of the proof.

To construct $\lambda_{\mathfrak{n}}$ and $\rho_{\mathfrak{n}}$\,, we recall that we can represent a pairing $\mathfrak{n}$ in $P_2(2T)$ by
\begin{equation*}
\{\mathfrak{n}(1), \mathfrak{n}(2)\} \{\mathfrak{n}(3), \mathfrak{n}(4)\} \cdots \{\mathfrak{n}(2T-1), \mathfrak{n}(2T)\}\,.
\end{equation*}
Let us partition the individual pairs $\{\mathfrak{n}(2k-1), \mathfrak{n}(2k)\}$ into three families:
\begin{align}
\mathcal{F}_{\text{I,I}} &= \big\{\{\mathfrak{n}(2k-1), \mathfrak{n}(2k)\} \in \mathfrak{n} \, : \, \mathfrak{n}(2k-1),\mathfrak{n}(2k)  \text{ are odd}\big\} \\
\mathcal{F}_{\text{II,II}} &= \big\{\{\mathfrak{n}(2k-1), \mathfrak{n}(2k)\} \in \mathfrak{n} \, : \, \mathfrak{n}(2k-1),\mathfrak{n}(2k) \text{ are even} \big\} \\
\mathcal{F}_{\text{I,II}} &= \big\{\{\mathfrak{n}(2k-1), \mathfrak{n}(2k)\} \in \mathfrak{n} \, : \,  \text{one of }\mathfrak{n}(2k-1),\,\mathfrak{n}(2k) \text{ is odd, the other is even} \big\}\,.
\end{align}
For convenience, we prescribe an ordering for the elements in these sets.  We write
\begin{align}
\mathcal{F}_{\text{I,I}} &=\big\{\{a_1, a_1'\},\,\{a_2,a_2'\},...\{a_{M}, a_{M}'\} \} \\
\mathcal{F}_{\text{II,II}} &= \{\{b_1, b_1'\},\,\{b_2, b_2'\},...\{b_{M}, b_{M}'\} \}  \\
\mathcal{F}_{\text{I,II}} &= \{\{c_1, c_1'\},\,\{c_2, c_2'\},...\{c_{T - 2M}, c_{T - 2M}'\} \} 
\end{align}
where we impose:
\begin{enumerate}
\item $a_k < a_k'$ and $b_k < b_k'$.
\item The pairs within $\mathcal{F}_{\text{I,I}}$ are ordered according to $a_1 < a_2 < \cdots$.
\item Each $c_k$ is odd and each $c_k'$ is even. (Note that $c_k$ need not be less than $c_k'$).
\item Suppose $\{a_k, a_k'\}$ for some fixed $k$ belongs to the $M_{\text{2T}}$-cycle $B_j$.  Each $B_j$ is cyclically ordered, but we can fix the order by mandating that the first element is the smallest integer appearing in the cycle.  Thus we have turned $B_k$ into an ordered list, which can be regarded as a list of pairs of the form $\{i, \mathfrak{n}(i)\}$.  Suppose that $\{a_k, a_k'\}$ is the $\ell$th appearance of a pair in $\mathcal{F}_{\text{I,I}}$ on the list $B_j$.  Then let $\{b_k, b_k'\}$ be the pair which is the $\ell$th appearance of a pair in $\mathcal{F}_{\text{II,II}}$ on the list $B_j$.
\item The pairs within $\mathcal{F}_{\text{I,II}}$ are ordered according to $\text{min}(c_1, c_1') < \text{min}(c_2,c_2') < \cdots$\,.
\end{enumerate}
Now we are equipped to construct $\lambda_{\mathfrak{n}}, \mathfrak{\rho}_{\mathfrak{n}} \in S_{T}$.  They are defined by
\begin{align}
(\rho_{\mathfrak{n}}(1), \rho_{\mathfrak{n}}(2),..., \rho_{\mathfrak{n}}(T) ) &= \left(\frac{a_1+1}{2}, \frac{a_1'+1}{2},...,\frac{a_{|\mathcal{F}_{\text{I,I}}|}+1}{2},\frac{a_{|\mathcal{F}_{\text{I,I}}|}'+1}{2}, \frac{c_1+1}{2}, \frac{c_2+1}{2},..., \frac{c_{|\mathcal{F}_{\text{I,II}}|} + 1}{2}\right)  \\
(\lambda_{\mathfrak{n}}(1), \lambda_{\mathfrak{n}}(2),..., \lambda_{\mathfrak{n}}(T) ) &= \left(\frac{b_1}{2}, \frac{b_1'}{2}, ...,\frac{b_{|\mathcal{F}_{\text{II,II}}|}}{2},\frac{b_{|\mathcal{F}_{\text{II,II}}|}'}{2}, \frac{c_1'}{2}, \frac{c_2'}{2},..., \frac{c_{|\mathcal{F}_{\text{I,II}}|}'}{2} \right) \,.
\end{align}
It will be convenient to define
\begin{align}
\widetilde{a}_k := \frac{a_k+1}{2}\,, \quad \widetilde{a}_k' := \frac{a_k'+1}{2}\,,\quad \widetilde{b}_k := \frac{b_k}{2}\,, \quad \widetilde{b}_k' := \frac{b_k'}{2}\,,\quad \widetilde{c}_k := \frac{c_k + 1}{2}\,,\quad \widetilde{c}_k' := \frac{c_k'}{2}
\end{align}
to ease notation.

Recall that a fixed pair permutation $\mathfrak{n}$ can be decomposed into $M_{2T}$-cycles $B_1 B_2 \cdots B_{\#^O(\mathfrak{n})}$.  We will say that $i \leftrightarrow j$ is in the $m$th cycle $B_m$ if $B_m = (\cdots ij \cdots)$.  Then for fixed $\mathfrak{n} = B_1 B_2 \cdots B_{\#^O(\mathfrak{n})}$ and letting $v_0 = r, v_1,...,v_{T-1}, v_T = \ell$ be the root-to-leaf path terminating in $\ell$, the following lemma holds:
\begin{lemma}
    We have the following identity:
    \begin{align}
    \label{E:Ocycledecomp1}
        \includegraphics[scale=.32, valign = c]{Ocycledecomp1.pdf}
    \end{align}
\end{lemma}

\begin{proof}
Consider a $M_{2T}$-cycle $C_m$ of $\mathfrak{n}$, and some $a_k \leftrightarrow a_k' \in B_m$ where $k$ is fixed. The solid leg of $| \phi_{v_{\widetilde{a}_k - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{a}_k}}\rangle$.  Likewise the solid leg of $| \phi_{v_{\widetilde{a}_k' - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{a}_k'}}\rangle$.  The solid leg of $|\psi_{v_{\widetilde{a}_k}}\rangle$ is connected to the solid leg of $|\psi_{v_{\widetilde{a}_k'}}\rangle$ via an unnormalized maximally entangled state.

By our ordering and labeling conventions, $b_k \leftrightarrow b_k'$ (for the same $k$ as in $a_k \leftrightarrow a_k'$ above) is also in $B_m$.  We similarly have that the solid leg of $| \phi_{v_{\widetilde{b}_k - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{b}_k}}\rangle$.  Likewise the solid leg of $| \phi_{v_{\widetilde{b}_k' - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{b}_k'}}\rangle$.  Finally the solid leg of $|\psi_{v_{\widetilde{b}_k}}\rangle$ is connected to the solid leg of $|\psi_{v_{\widetilde{b}_k'}}\rangle$ via an unnormalized maximally entangled state.

Next we turn to the $c_k \leftrightarrow c_k'$ pairs.  The solid legs of $\langle \phi_{v_{\widetilde{c}_k'-1}}|$ and $|\phi_{v_{\widetilde{c}_k-1}}\rangle$ are dangling.  The dotted leg of $\langle \psi_{v_{\widetilde{c}_k'-1}}|$ connects to the dotted leg of $\ket{\psi_{v_{\widetilde{c}_k'}}}$, and the dotted leg of $|\psi_{v_{\widetilde{c}_k-1}}\rangle$ connects to the dotted leg of $\ket{\psi_{v_{\widetilde{c}_k'}}}$.  Lastly, the solid leg of $\langle \psi_{v_{\widetilde{c}_k'}}|$ is connected to the solid leg of $|\psi_{v_{\widetilde{c}_k}}\rangle$.

The above accounts for all legs among $\phi_{v_{i-1}}$, $\psi_{v_i}$, $\phi_{v_{j - 1}}$, and $\psi_{v_j}$, which yields the stated lemma.  Figure~\ref{fig:O_example_cycledecomp} depicts a representative example. \TODO{}
    \begin{figure}[h]\label{fig:O_example_cycledecomp}
        \caption{\color{red} {[example illustration of the decomposition for alphabet size 2 or 3, TODO]}}
    \end{figure}
\end{proof}

Next we will convert~\eqref{E:Ocycledecomp1} into a product of traces. For any $i\in[T]$, define the unnormalized density operator $\widetilde{\rho}_{v_i} \in \text{Mat}_{d \times d}(\mathbb{C})$ by
\begin{align}
\label{E:rhotildedef}
    \includegraphics[scale=.32, valign = c]{rhotildedef.png}
\end{align}

\begin{lemma}
We say that two integers $i,j \in [2T]$ have the same parity if they are both odd or both even, and that they have opposities parities of one is even and the other is odd.  For any $i\leftrightarrow j\in B_m$, the corresponding term on the right-hand side of \eqref{E:Ocycledecomp1} is upper bounded by $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})$ if $i,j$ have oppositive parities, and $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j}^{\,t})$ if $i,j$ have the same parity. Then \eqref{E:Ocycledecomp1} upper bounded by
\begin{equation}\label{E:Oproductwithsqrt1}
        \prod^{\#^O(\mathfrak{n})}_{m = 1}\left(\prod_{\substack{i\leftrightarrow j\in B_m \\ i,j\,\,\text{\rm opposite parity}}} \sqrt{\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})} \prod_{\substack{k\leftrightarrow \ell\in B_m \\ k,\ell\,\,\text{\rm same parity}}} \sqrt{\Tr(\wt{\rho}_{v_k}\wt{\rho}_{v_\ell}^{\,t})}\right)\,.
    \end{equation}
\end{lemma}

\begin{proof}
If $i,j$ have opposite parity, they correspond to a pair $c_k \leftrightarrow c_k' \in B_m$.  Considering the right-most product in~\eqref{E:Ocycledecomp1}, we use $\|A\|_1 = \|A\otimes A^\dagger\|_1^{1/2} \leq \|\text{SWAP}  \cdot (A\otimes A^\dagger)\|_1^{1/2}$ to find
\begin{align}
    \includegraphics[scale=.32, valign = c]{SWAPineq1.png} \nonumber
\end{align}
Since the tensor network in the trace is positive semi-definite, we can compute the 1-norm by taking to trace and find
\begin{align}
\label{E:O1normproperty2}
\includegraphics[scale=.32, valign = c]{O1normproperty2.pdf}
\end{align}
We have colored the tensor diagram suggestively so that it is transparent how to rewrite it as $\sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})}$.

On the other hand, if $k, \ell$ have opposite parities, they correspond to either a term $a_k \leftrightarrow a_k' \in B_m$ or a term $b_k \leftrightarrow b_k'$ in $B_m$.  Accordingly, consider a term in the $\prod_{\substack{a_k \leftrightarrow a_k' \in B_m \\ b_k \leftrightarrow b_k' \in B_m}}$ product on the right-hand side of~\eqref{E:Ocycledecomp1}.  Using the identity $\||\varphi\rangle \langle \varphi'| \|_1 = \sqrt{\langle \varphi|\varphi\rangle} \sqrt{\langle \varphi'|\varphi'\rangle}$ we find 
\begin{align}
\label{E:O1normproperty3}
\includegraphics[scale=.32, valign = c]{O1normproperty3.pdf}
\end{align}
We have colored the right-hand side to show how it is equivalent to
\begin{equation}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{\widetilde{a}_k}} \widetilde{\rho}_{v_{\widetilde{a}_k'}}^{\,t})} \, \sqrt{\text{tr}(\widetilde{\rho}_{v_{\widetilde{b}_k}} \widetilde{\rho}_{v_{\widetilde{b}_k'}}^{\,t})} \,.
\end{equation}

The lemma follows by taking the products over $\sqrt{\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})}$ and $\sqrt{\Tr(\wt{\rho}_{v_k}\wt{\rho}_{v_\ell}^{\,t})}$ for $i \leftrightarrow j \in B_m$ having opposite parity and $k \leftrightarrow \ell \in B_m$ having the same parity, and then taking a product over $M_{2T}$ cycles of $\mathfrak{n}$.

\end{proof} 

Now we turn to bounding~\eqref{E:Oproductwithsqrt1}.  We begin by developing some notation for cycles $B_m$\,.  Standard notation for an $M_{2T}$ cycle of length $p$ is $B_m = (a_1 a_2 \cdots a_p)$ where for us $\{a_1, a_2,...,a_p\} \subseteq  [2T]$.  We decorate each $a_i$ by an additional subscript as $a_{m,i}$ to remember that it that belongs to the $m$th cycle $B_m$. We sometimes write $p = |B_m|$ to remind ourselves that it depends on $m$.  Let us also define
\begin{align}
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}^{\,t(i,j)}) := \begin{cases}
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}) & \text{if }i,j\text{ have different parities}\\
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}^{\,t}) & \text{if }i,j\text{ have the same parity}\\
\end{cases}\,.
\end{align}
With these notations in mind, we can write~\eqref{E:Oproductwithsqrt1} as a product over
\begin{equation}
\label{E:Ocycletobound1}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}} \widetilde{\rho}_{v_{a_{m,2}}}^{\,t(a_{m,1}, a_{m,2})})}  \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,2}}} \widetilde{\rho}_{v_{a_{m,3}}}^{\,t(a_{m,2}, a_{m,3})})} \,\cdots \, \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p-1}}} \widetilde{\rho}_{v_{a_{m,p}}}^{\,t(a_{m,p-1}, a_{m,p})})} \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}}^{\,t(a_{m,p}, a_{m,p-1})})}
\end{equation}
over $m = 1, \ldots, \#^O(\mathfrak{n})$.
We will further analyze the above for fixed $m$ in two cases: (i) $p = |B_m|$ is even, and (ii) $p = |B_m|$ is odd. \\ \\
\textcolor{red}{[NEED TO FIX]}
\textbf{Case 1:} \textit{$p$ is even.} Each term in Eqn.~\eqref{E:Ocycletobound1} has the form $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}$ except for the last term; however, if we treat the $i$ subscripts of $a_{m,i}$ modulo $p$, then we can write the last term as $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,p+1}}})}$\,.  We elect to use this notation.  Then we can rearrange and group the terms in Eqn.~\eqref{E:cycletobound1} as follows
\begin{equation}
\left(\prod_{i\text{ odd}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, the above is upper bounded by
\begin{equation}
\frac{1}{2} \prod_{i\text{ odd}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})\,.
\end{equation}
We will call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. \\ \\
\textbf{Case 2:} \textit{$p$ is odd.} Again consider the product in Eqn.~\eqref{E:cycletobound1}.  We can rearrange and group terms as
\begin{equation}
\label{E:oddsplit1}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})}\left(\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
If two matrices $A,B$ are Hermitian and positive semi-definite, then using Cauchy-Schwarz combined with operator norm inequalities we have $\text{tr}(AB) \leq \|A\|_2 \, \|B\|_2 \leq \|A\|_1 \, \|B\|_1 \leq \text{tr}(A) \, \text{tr}(B)$.  Accordingly, we have $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})} \leq \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}}) \, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}$ and so~\eqref{E:oddsplit1} is upper bounded by
\begin{equation}
\left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})} \prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Again using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, we have the upper bound
\begin{equation}
\frac{1}{2} \,\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})
\end{equation}
where we analogously call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. 

In both cases, note that $R_{m,\,-}$ and $R_{m,\,+}$ implicitly depend on the leaf $\ell$, so we will denote them by $R^{\ell}_{m,\,-}$ and $R^{\ell}_{m,\,+}$ when we wish to make this dependence explicit.\\ \\
\indent Putting together our notation and bounds from Case 1 and Case 2, we find that Eqn.~\eqref{E:productwithsqrt1} is upper bounded by
\begin{align}
\label{E:multipleTs}
\prod_{m=1}^{\#(\tau^{-1})} \,\prod_{i \to j \, \in C_m} \sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})} &\leq \frac{1}{2^{\#(\tau^{-1})}} \prod_{m=1}^{\#(\tau^{-1})} \left(R_{m,-} + R_{m,+} \right) \nonumber \\
&= \frac{1}{2^{\#(\tau^{-1})}} \sum_{i_1,...,i_{\#(\tau^{-1})} = \pm} R_{1,i_1} R_{2,i_2} \cdots R_{\#(\tau^{-1}), i_{\#(\tau^{-1})}}\,.
\end{align}
Each term in the sum in the last line of~\eqref{E:multipleTs} is a product of terms like $\text{tr}(\widetilde{\rho}_{v_i})$ and $\text{tr}(\widetilde{\rho}_{v_j} \widetilde{\rho}_{v_k})$.  But the key point is that we have arranged the equations so that each term in the sum has $\widetilde{\rho}_{v_i}$ for each $i = 1,...,T$ appear \textit{exactly once}.  This has the following highly useful consequence.


\begin{lemma}\label{lem:collapse}
    Fix any $i_1,...,i_{\#(\tau^{-1})} \in \{+,-\}$. Then
    \begin{equation}
        \label{E:sboundhard1}
        \sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} (d d')^T \,W_\ell \, R^{\ell}_{1,i_1} R^{\ell}_{2,i_2} \cdots R^{\ell}_{\#(\tau^{-1}), i_{\#(\tau^{-1})}} \le d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2}\right\rfloor}
    \end{equation}
where $L(\tau^{-1})$ is the length of the longest cycle in $\tau^{-1}$.
\end{lemma}

\begin{proof}
    For ease of notation, we will let $R^{\ell}_j\triangleq R^{\ell}_{j,i_j}$.
    Recall from~\eqref{E:Wbig1} that $W_\ell = w_{v_1} w_{v_2} \cdots w_{v_T}$ and note that
    \begin{equation}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \widetilde{\rho}_{v} = \langle \phi_{\text{parent}(v)} | \phi_{\text{parent}(v)}\rangle\, \mathds{1}_{d \times d} = \mathds{1}_{d \times d}\,.
    \end{equation}
    Accordingly we have that for any $\rho\in\text{Mat}_{d\times d}(\mathbb{C})$,
    \begin{align}
        \label{E:2tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\, w_{v} \, \text{tr}(\widetilde{\rho}_{v} \, \rho ) = \text{tr}(\rho)\,,
    \end{align}
    and in particular, for $\rho = \mathds{1}$,
    \begin{align}
        \label{E:1tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \text{tr}(\widetilde{\rho}_{v}) &= d.
    \end{align}
    We now turn to bounding the left-hand side of \eqref{E:sboundhard1}. Recalling that $\prod_j R^{\ell}_j$ as a product of terms like $\Tr(\wt{\rho}_{v_i})$ and $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_i'})$, we will define some sets of indices encoding this data. Let $S^{(T)}_1\subseteq[T]$ denote the indices $i$ for which $\Tr(\wt{\rho}_{v_i})$ appears in $\prod_j R^{\ell}_j$, and let $S^{(T)}_2\subseteq[T]\times[T]$ denote the set of (unordered) pairs $(i,i')$ for which $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})$ appears, so that for any root-to-leaf path in $\calT$ consisting of nodes $v_1,\ldots,v_T = \ell$, we have
    \begin{equation}
        \label{eq:prodRs}
        \prod_j R^{\ell}_j = \prod_{i\in S^{(T)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i')\in S^{(T)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})
    \end{equation} by definition. Now construct $S^{(t)}_1\subseteq[t]$ and $S^{(t)}_2\subseteq[t]\times[t]$ for $1 \le t < T$ inductively as follows. If $t\in S^{(t)}_1$ then define $S^{(t-1)}_1 \triangleq S^{(t)}_1 \backslash \brc{t}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2$. Otherwise if $(t,t')\in S^{(t)}_2$ for some $t' < t$, then define $S^{(t-1)}_1 \triangleq S^{(t-1)}_1 \cup \brc{t'}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2 \backslash \brc{(t,t')}$. We collect some basic observations about these two set sequences:
    
    \begin{observation}\label{obs:singleton}
        For every $i\in S^{(T)}_1$, we have that $i\in S^{(i)}_1$.
    \end{observation}
    
    \begin{observation}\label{obs:pair}
        For every $(i,i')\in S^{(T)}_2$, if $i\le i'$ then $i\in S^{(i)}_1$ while $i'\not\in S^{(i')}_1$.
    \end{observation}
    
    The reason for defining these set sequences is that we can extract $\wt{\rho}_{v_T}$ from the product on the right-hand side of \eqref{eq:prodRs} and apply \eqref{E:1tracebound1} (resp. \eqref{E:2tracebound1}) if $T\in S^{(T)}_1$ (resp. $(T,t')\in S^{(T)}_2$ for some $t' < T$) to obtain \begin{equation}
        \label{eq:induct_prodRs}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j = d^{\bone{T\in S^{(T)}_1}}\sum_{u: \,\text{depth}(u) = T - 1} (dd')^{T-1} W_u \prod_{i\in S^{(T-1)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i') \in S^{(T-1)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}}),
    \end{equation} where $W_u = w_{v_1}\cdots w_{v_{T-1}}$ if the path from root to $u$ in $\calT$ consists of $v_1,\ldots,v_{T-1} = u$.
    Proceeding inductively, we can express the right-hand side of \eqref{eq:induct_prodRs} as \begin{equation}
        d^{\sum^T_{t=1} \bone{t\in S^{(t)}_1}}.
    \end{equation} By Observations~\ref{obs:singleton} and \ref{obs:pair}, $\sum^T_{t=1}\bone{t\in S^{(t)}_1} = |S^{(T)}_1| + |S^{(T)}_2|$. Because every even cycle $C_m$ of $\tau^{-1}$ contributes $|C_m|/2$ pairs to $S^{(T)}_2$, and every odd cycle $C_m$ contributes $\floor{|C_m|/2}$ pairs to $S^{(T)}_2$ and one element to $S^{(T)}_1$, we conclude that
    \begin{align}
        \label{E:sboundhard2}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j &= d^{\sum_{m=1}^{\#(\tau^{-1})} \left\lceil \frac{|C_m|}{2} \right\rceil} \nonumber \\
        &= d^{\frac{T}{2} - \sum_{m=1}^{\#(\tau^{-1})} \left\lfloor \frac{|C_m|}{2} \right\rfloor} \nonumber \\
        &\leq d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2} \right\rfloor}
    \end{align}
    as claimed.
\end{proof}
\textcolor{red}{[END OF PARTS WE NEED TO FIX]}
    
Putting all our previous bounds together, in particular Eq.~\eqref{E:Othirdterm1},~\eqref{E:OHolder2},~\eqref{E:Othirdterm1},~\eqref{E:Ocycledecomp1},~\eqref{E:Oproductwithsqrt1},~\eqref{E:multipleTs},~\eqref{E:sboundhard1}, we arrive at
\begin{equation}
\sum_{\ell \, \in \, \text{leaf}(\mathcal{T})} \sum_{\mathfrak{n} \not = \mathfrak{e}, \,\mathfrak{m}}|p_{\sigma, \tau}^{\mathcal{O}}(\ell)| \leq d^{T} \sum_{\mathfrak{m}} |\text{Wg}^O(\sigma_{\mathfrak{m}}^{-1}, d)| \sum_{\mathfrak{n} \not = \mathfrak{e}} d^{- \left\lfloor \frac{L^O(\mathfrak{n})}{4} \right\rfloor} \,.
\end{equation}
The first sum on the right-hand side is bounded by $d^T \sum_{\mathfrak{m}} |\text{Wg}^O(\sigma_{\mathfrak{m}}^{-1}, d)| \leq 1 + \mathcal{O}\!\left( \frac{T^2}{d}\right)$.  Considering the second sum on the right-hand side, let $N^O(T,\ell)$ be the number of permutations in $S_T$ where the length of the longest $M_{2T}$-cycle is $2\ell$.  Then the second sum can be written as
\begin{equation}
\label{E:sumNTell}
\sum_{\ell = 2}^T N^O(T,\ell) \, d^{- \left\lfloor \frac{\ell}{2} \right\rfloor}
\end{equation}
where we omit $\ell = 1$ from the sum since it corresponds to the identity pair permutation.  Since $N^O(T,\ell) \leq \binom{2T}{2\ell}(2\ell - 1)!! = \frac{(2T)!}{(2T - 2\ell)! \,2^\ell \ell!} < T^\ell$,~\eqref{E:sumNTell} is upper bounded by
\begin{equation}
\sum_{\ell = 2}^\infty T^\ell  \, d^{- \left\lfloor \frac{\ell}{2} \right\rfloor} = \frac{(1 + T) \frac{T^2}{d}}{1 - \frac{T^2}{d}} = \frac{T^3}{d} + \frac{T^2}{d} + \mathcal{O}\!\left(\frac{T^5}{d^2}\right)\,.
\end{equation}
%we observe that the number of permutations of $T$ items with $L$ disjoint cycles (including counting cycles of unit length) is given by the unsigned Stirling numbers of the first kind ${ T\brack L}$.  As such we can write
%\begin{equation}
%\label{E:1stirling1}
%\sum_{\tau \not = \mathds{1}} d^{\#(\tau^{-1})/2}  = \sum_{L=0}^{T-1} { T\brack L}  d^{L/2} 
%\end{equation}
%where we only sum up to $T-1$ since $L = T$ corresponds to $\tau^{-1} = \mathds{1}$ which is omitted from the sum.  Unsigned Stirling numbers of the first kind enjoy the identity $\sum_{L=0}^T { T\brack L} \, x^L = x (x+1) \cdots (x + T - 1)$ and so~\eqref{E:1stirling1} is equivalent to
%\begin{align}
%d^{1/2} \left(d^{1/2}  + 1\right) \cdots \left(d^{1/2}  + T-1 \right) - d^{T/2} &\le d^{T/2}\left(\exp\left(\frac{T(T-1)}{d^{1/2}}\right) - 1\right).
%\end{align}
Now if $T \le o(d^{1/3})$, then this quantity is $o(1)$ for some absolute constant $c > 0$. Altogether, we find
\begin{equation}
\frac{1}{2}\sum_{\ell\,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{n}\not = \mathfrak{e}, \,\mathfrak{m}}|p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{O}}(\ell)| \leq o\!\left(1\right)\,.
\end{equation}
% \\ \\
% \indent In totality, for $T \leq \frac{\sqrt{d}}{4}$ we find
% \begin{equation}
% \frac{1}{2}\sum_s |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)]| \leq o\!\left(1\right)
% \end{equation}
% which is the claimed result.

\subsubsection*{Third term for \normalfont $\text{Sp}(d/2)$ \normalfont \textbf{case}}
The third term in~\eqref{E:Spfirstineq1} is $\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{n} \not = \mathfrak{e}, \,\mathfrak{m}}|p_{\mathfrak{m},\mathfrak{n}}^{\mathcal{S}}(\ell)|$.  Applying the Cauchy-Schwarz inequality we obtain the upper bound
\begin{align}
\label{E:Spthirdterm1}
    \includegraphics[scale=.32, valign = c]{Othirdterm1.pdf}
\end{align}
Similar to above, we can upper bound the diagrammatic term using the H\"{o}lder inequality as
\begin{align}
\label{E:SpHolder2}
    \includegraphics[scale=.32, valign = c]{SpHolder2.pdf}
\end{align}
where we have similarly used $\|\Delta_{\mathfrak{m}}'\|_\infty = \|\textbf{J}^t\|_\infty = 1$.  Letting $\lambda_{\mathfrak{n}}$ and $\rho_{\mathfrak{n}}$ be the permutations on $S_{T}$ that we will specified in the orthogonal setting above, we use the H\"{o}lder inequality to obtain
\begin{align}
\includegraphics[scale=.32, valign = c]{Sptensorreorder1.pdf}
\end{align}
where we have used $\|\lambda_{\mathfrak{n}}^{-1}\|_\infty = \|\rho_{\mathfrak{n}}\|_\infty = 1$. 

Recall that a fixed pair permutation $\mathfrak{n}$ can be decomposed into $M_{2T}$-cycles $B_1 B_2 \cdots B_{\#^O(\mathfrak{n})}$.  We will say that $i \leftrightarrow j$ is in the $m$th cycle $B_m$ if $B_m = (\cdots ij \cdots)$.  Then for fixed $\mathfrak{n} = B_1 B_2 \cdots B_{\#^O(\mathfrak{n})}$ and letting $v_0 = r, v_1,...,v_{T-1}, v_T = \ell$ be the root-to-leaf path terminating in $\ell$, the following lemma holds:
\begin{lemma}
    We have the following identity:
    \begin{align}
    \label{E:Spcycledecomp1}
        \includegraphics[scale=.32, valign = c]{Spcycledecomp1.pdf}
    \end{align}
\end{lemma}

\begin{proof}
Consider a $M_{2T}$-cycle $C_m$ of $\mathfrak{n}$, and some $a_k \leftrightarrow a_k' \in B_m$ where $k$ is fixed. The solid leg of $| \phi_{v_{\widetilde{a}_k - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{a}_k}}\rangle$.  Likewise the solid leg of $| \phi_{v_{\widetilde{a}_k' - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{a}_k'}}\rangle$.  The solid leg of $|\psi_{v_{\widetilde{a}_k}}\rangle$ is connected to the solid leg of $|\psi_{v_{\widetilde{a}_k'}}\rangle$ via an unnormalized maximally entangled state.

By our ordering and labeling conventions, $b_k \leftrightarrow b_k'$ (for the same $k$ as in $a_k \leftrightarrow a_k'$ above) is also in $B_m$.  We similarly have that the solid leg of $| \phi_{v_{\widetilde{b}_k - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{b}_k}}\rangle$.  Likewise the solid leg of $| \phi_{v_{\widetilde{b}_k' - 1}}\rangle$ is dangling and the dotted leg connects to $|\psi_{v_{\widetilde{b}_k'}}\rangle$.  Finally the solid leg of $|\psi_{v_{\widetilde{b}_k}}\rangle$ is connected to the solid leg of $|\psi_{v_{\widetilde{b}_k'}}\rangle$ via an unnormalized maximally entangled state and an insertion of a $\textbf{J}$ (on account of the definition of $\Delta_{\mathfrak{n}}'$).

Next we turn to the $c_k \leftrightarrow c_k'$ pairs.  The solid legs of $\langle \phi_{v_{\widetilde{c}_k'-1}}|$ and $|\phi_{v_{\widetilde{c}_k-1}}\rangle$ are dangling.  The dotted leg of $\langle \psi_{v_{\widetilde{c}_k'-1}}|$ connects to the dotted leg of $\ket{\psi_{v_{\widetilde{c}_k'}}}$, and the dotted leg of $|\psi_{v_{\widetilde{c}_k-1}}\rangle$ connects to the dotted leg of $\ket{\psi_{v_{\widetilde{c}_k'}}}$.  Lastly, the solid leg of $\langle \psi_{v_{\widetilde{c}_k'}}|$ is connected to the solid leg of $|\psi_{v_{\widetilde{c}_k}}\rangle$; a \textbf{J} is inserted along this leg due to the definition of $\Delta_{\mathfrak{n}}'$.

The above accounts for all legs among $\phi_{v_{i-1}}$, $\psi_{v_i}$, $\phi_{v_{j - 1}}$, and $\psi_{v_j}$, which yields the stated lemma.  Figure~\ref{fig:O_example_cycledecomp} depicts a representative example. \TODO{}
    \begin{figure}[h]\label{fig:O_example_cycledecomp}
        \caption{\color{red} {[example illustration of the decomposition for alphabet size 2 or 3, TODO]}}
    \end{figure}
\end{proof}

Next we will convert~\eqref{E:Ocycledecomp1} into a product of traces. For any $i\in[T]$, define the unnormalized density operator $\widetilde{\rho}_{v_i} \in \text{Mat}_{d \times d}(\mathbb{C})$ by
\begin{align}
\label{E:rhotildedef}
    \includegraphics[scale=.32, valign = c]{rhotildedef.png}
\end{align}
and recall that the symplectic transpose is defined by $A^D := J A^t J^{-1}$.

\begin{lemma}
We say that two integers $i,j \in [2T]$ have the same parity if they are both odd or both even, and that they have opposities parities of one is even and the other is odd.  For any $i\leftrightarrow j\in B_m$, the corresponding term on the right-hand side of \eqref{E:Ocycledecomp1} is upper bounded by $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})$ if $i,j$ have oppositive parities, $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j}^{\,t})$ if $i,j$ are both odd, and $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j}^{\,D})$ if $i,j$ are both even. Then \eqref{E:Ocycledecomp1} upper bounded by
\begin{equation}\label{E:Oproductwithsqrt1}
        \prod^{\#^O(\mathfrak{n})}_{m = 1}\left(\prod_{\substack{i\leftrightarrow j\in B_m \\ i,j\,\,\text{\rm opposite parity}}} \sqrt{\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})} \prod_{\substack{k\leftrightarrow \ell\in B_m \\ k,\ell\,\,\text{\rm both odd}}} \sqrt{\Tr(\wt{\rho}_{v_k}\wt{\rho}_{v_\ell}^{\,t})} \prod_{\substack{p\leftrightarrow q\in B_m \\ p,q\,\,\text{\rm both even}}} \sqrt{\Tr(\wt{\rho}_{v_p}\wt{\rho}_{v_q}^{\,D})}\right)\,.
    \end{equation}
\end{lemma}

\begin{proof}
If $i,j$ have opposite parity, they correspond to a pair $c_k \leftrightarrow c_k' \in B_m$.  Considering the right-most product in~\eqref{E:Ocycledecomp1}, we use $\|A\|_1 = \|A\otimes A^\dagger\|_1^{1/2} \leq \|\text{SWAP}  \cdot (A\otimes A^\dagger)\|_1^{1/2}$ to find
\begin{align}
    \includegraphics[scale=.32, valign = c]{SWAPineq1.png} \nonumber
\end{align}
Since the tensor network in the trace is positive semi-definite, we can compute the 1-norm by taking to trace and find
\begin{align}
\label{E:Sp1normproperty2}
\includegraphics[scale=.32, valign = c]{O1normproperty2.pdf}
\end{align}
We have colored the tensor diagram suggestively so that it is transparent how to rewrite it as $\sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})}$.

On the other hand, if $k, \ell$ have opposite parities, they correspond to either a term $a_k \leftrightarrow a_k' \in B_m$ or a term $b_k \leftrightarrow b_k'$ in $B_m$.  Accordingly, consider a term in the $\prod_{\substack{a_k \leftrightarrow a_k' \in B_m \\ b_k \leftrightarrow b_k' \in B_m}}$ product on the right-hand side of~\eqref{E:Ocycledecomp1}.  Using the identity $\||\varphi\rangle \langle \varphi'| \|_1 = \sqrt{\langle \varphi|\varphi\rangle} \sqrt{\langle \varphi'|\varphi'\rangle}$ we find 
\begin{align}
\label{E:O1normproperty3}
\includegraphics[scale=.32, valign = c]{Sp1normproperty2.pdf}
\end{align}
We have colored the right-hand side to show how it is equivalent to
\begin{equation}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{\widetilde{a}_k}} \widetilde{\rho}_{v_{\widetilde{a}_k'}}^{\,t})} \, \sqrt{\text{tr}(\widetilde{\rho}_{v_{\widetilde{b}_k}} \widetilde{\rho}_{v_{\widetilde{b}_k'}}^{\,D})} \,.
\end{equation}

The lemma follows by taking the products over $\sqrt{\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_j})}$, $\sqrt{\Tr(\wt{\rho}_{v_k}\wt{\rho}_{v_\ell}^{\,t})}$, and $\sqrt{\Tr(\wt{\rho}_{v_p}\wt{\rho}_{v_q}^{\,D})}$ for $i \leftrightarrow j \in B_m$ having opposite parity, $k \leftrightarrow \ell \in B_m$ with $k,\ell$ even, $p \leftrightarrow q \in B_m$ with $p,q$ odd, and finally taking a product over $M_{2T}$ cycles of $\mathfrak{n}$.

\end{proof} 

Now we turn to bounding~\eqref{E:Oproductwithsqrt1}.  We begin by developing some notation for cycles $B_m$\,.  Standard notation for an $M_{2T}$ cycle of length $p$ is $B_m = (a_1 a_2 \cdots a_p)$ where for us $\{a_1, a_2,...,a_p\} \subseteq  [2T]$.  We decorate each $a_i$ by an additional subscript as $a_{m,i}$ to remember that it that belongs to the $m$th cycle $B_m$. We sometimes write $p = |B_m|$ to remind ourselves that it depends on $m$.  Let us also define
\begin{align}
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}^{\,D(i,j)}) := \begin{cases}
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}) & \text{if }i,j\text{ have different parities}\\
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}^{\,t}) & \text{if }i,j\text{ are both odd}\\
\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j}^{\,D}) & \text{if }i,j\text{ are both even}\\
\end{cases}\,.
\end{align}
With these notations in mind, we can write~\eqref{E:Oproductwithsqrt1} as a product over
\begin{equation}
\label{E:Ocycletobound1}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}} \widetilde{\rho}_{v_{a_{m,2}}}^{\,D(a_{m,1}, a_{m,2})})}  \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,2}}} \widetilde{\rho}_{v_{a_{m,3}}}^{\,D(a_{m,2}, a_{m,3})})} \,\cdots \, \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p-1}}} \widetilde{\rho}_{v_{a_{m,p}}}^{\,D(a_{m,p-1}, a_{m,p})})} \,  \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}}^{\,D(a_{m,p}, a_{m,p-1})})}
\end{equation}
over $m = 1, \ldots, \#^{\text{Sp}}(\mathfrak{n})$.
We will further analyze the above for fixed $m$ in two cases: (i) $p = |B_m|$ is even, and (ii) $p = |B_m|$ is odd. \\ \\
\textcolor{red}{[NEED TO FIX]}
\textbf{Case 1:} \textit{$p$ is even.} Each term in Eqn.~\eqref{E:Ocycletobound1} has the form $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}$ except for the last term; however, if we treat the $i$ subscripts of $a_{m,i}$ modulo $p$, then we can write the last term as $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,p+1}}})}$\,.  We elect to use this notation.  Then we can rearrange and group the terms in Eqn.~\eqref{E:cycletobound1} as follows
\begin{equation}
\left(\prod_{i\text{ odd}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, the above is upper bounded by
\begin{equation}
\frac{1}{2} \prod_{i\text{ odd}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})\,.
\end{equation}
We will call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. \\ \\
\textbf{Case 2:} \textit{$p$ is odd.} Again consider the product in Eqn.~\eqref{E:cycletobound1}.  We can rearrange and group terms as
\begin{equation}
\label{E:oddsplit1}
\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})}\left(\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
If two matrices $A,B$ are Hermitian and positive semi-definite, then using Cauchy-Schwarz combined with operator norm inequalities we have $\text{tr}(AB) \leq \|A\|_2 \, \|B\|_2 \leq \|A\|_1 \, \|B\|_1 \leq \text{tr}(A) \, \text{tr}(B)$.  Accordingly, we have $\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}} \widetilde{\rho}_{v_{a_{m,1}}})} \leq \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}}) \, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}$ and so~\eqref{E:oddsplit1} is upper bounded by
\begin{equation}
\left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})} \prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,i}}} \widetilde{\rho}_{v_{a_{m,i+1}}})}\right) \left(\sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})}\,\prod_{j\text{ even}} \sqrt{\text{tr}(\widetilde{\rho}_{v_{a_{m,j}}} \widetilde{\rho}_{v_{a_{m,j+1}}})}\right)\,.
\end{equation}
Again using the inequality $ab \leq \frac{1}{2}(a^2 + b^2)$, we have the upper bound
\begin{equation}
\frac{1}{2} \,\text{tr}(\widetilde{\rho}_{v_{a_{m,p}}})\prod_{\substack{i\text{ odd} \\ 1 \leq i \leq p - 2}} \text{tr}(\widetilde{\rho}_{v_{a_{i}}} \widetilde{\rho}_{v_{a_{i+1}}}) + \frac{1}{2}\, \text{tr}(\widetilde{\rho}_{v_{a_{m,1}}})\prod_{j\text{ even}} \text{tr}(\widetilde{\rho}_{v_{a_{j}}} \widetilde{\rho}_{v_{a_{j+1}}})
\end{equation}
where we analogously call the first term $\frac{1}{2}\,R_{m,\,-}$ and the second term $\frac{1}{2}\,R_{m,\,+}$\,. 

In both cases, note that $R_{m,\,-}$ and $R_{m,\,+}$ implicitly depend on the leaf $\ell$, so we will denote them by $R^{\ell}_{m,\,-}$ and $R^{\ell}_{m,\,+}$ when we wish to make this dependence explicit.\\ \\
\indent Putting together our notation and bounds from Case 1 and Case 2, we find that Eqn.~\eqref{E:productwithsqrt1} is upper bounded by
\begin{align}
\label{E:multipleTs}
\prod_{m=1}^{\#(\tau^{-1})} \,\prod_{i \to j \, \in C_m} \sqrt{\text{tr}(\widetilde{\rho}_{v_i} \widetilde{\rho}_{v_j})} &\leq \frac{1}{2^{\#(\tau^{-1})}} \prod_{m=1}^{\#(\tau^{-1})} \left(R_{m,-} + R_{m,+} \right) \nonumber \\
&= \frac{1}{2^{\#(\tau^{-1})}} \sum_{i_1,...,i_{\#(\tau^{-1})} = \pm} R_{1,i_1} R_{2,i_2} \cdots R_{\#(\tau^{-1}), i_{\#(\tau^{-1})}}\,.
\end{align}
Each term in the sum in the last line of~\eqref{E:multipleTs} is a product of terms like $\text{tr}(\widetilde{\rho}_{v_i})$ and $\text{tr}(\widetilde{\rho}_{v_j} \widetilde{\rho}_{v_k})$.  But the key point is that we have arranged the equations so that each term in the sum has $\widetilde{\rho}_{v_i}$ for each $i = 1,...,T$ appear \textit{exactly once}.  This has the following highly useful consequence.


\begin{lemma}\label{lem:collapse}
    Fix any $i_1,...,i_{\#(\tau^{-1})} \in \{+,-\}$. Then
    \begin{equation}
        \label{E:sboundhard1}
        \sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} (d d')^T \,W_\ell \, R^{\ell}_{1,i_1} R^{\ell}_{2,i_2} \cdots R^{\ell}_{\#(\tau^{-1}), i_{\#(\tau^{-1})}} \le d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2}\right\rfloor}
    \end{equation}
where $L(\tau^{-1})$ is the length of the longest cycle in $\tau^{-1}$.
\end{lemma}

\begin{proof}
    For ease of notation, we will let $R^{\ell}_j\triangleq R^{\ell}_{j,i_j}$.
    Recall from~\eqref{E:Wbig1} that $W_\ell = w_{v_1} w_{v_2} \cdots w_{v_T}$ and note that
    \begin{equation}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \widetilde{\rho}_{v} = \langle \phi_{\text{parent}(v)} | \phi_{\text{parent}(v)}\rangle\, \mathds{1}_{d \times d} = \mathds{1}_{d \times d}\,.
    \end{equation}
    Accordingly we have that for any $\rho\in\text{Mat}_{d\times d}(\mathbb{C})$,
    \begin{align}
        \label{E:2tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\, w_{v} \, \text{tr}(\widetilde{\rho}_{v} \, \rho ) = \text{tr}(\rho)\,,
    \end{align}
    and in particular, for $\rho = \mathds{1}$,
    \begin{align}
        \label{E:1tracebound1}
        \sum_{v: \, \text{depth}(v) = i} dd'\,w_{v} \, \text{tr}(\widetilde{\rho}_{v}) &= d.
    \end{align}
    We now turn to bounding the left-hand side of \eqref{E:sboundhard1}. Recalling that $\prod_j R^{\ell}_j$ as a product of terms like $\Tr(\wt{\rho}_{v_i})$ and $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_i'})$, we will define some sets of indices encoding this data. Let $S^{(T)}_1\subseteq[T]$ denote the indices $i$ for which $\Tr(\wt{\rho}_{v_i})$ appears in $\prod_j R^{\ell}_j$, and let $S^{(T)}_2\subseteq[T]\times[T]$ denote the set of (unordered) pairs $(i,i')$ for which $\Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})$ appears, so that for any root-to-leaf path in $\calT$ consisting of nodes $v_1,\ldots,v_T = \ell$, we have
    \begin{equation}
        \label{eq:prodRs}
        \prod_j R^{\ell}_j = \prod_{i\in S^{(T)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i')\in S^{(T)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}})
    \end{equation} by definition. Now construct $S^{(t)}_1\subseteq[t]$ and $S^{(t)}_2\subseteq[t]\times[t]$ for $1 \le t < T$ inductively as follows. If $t\in S^{(t)}_1$ then define $S^{(t-1)}_1 \triangleq S^{(t)}_1 \backslash \brc{t}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2$. Otherwise if $(t,t')\in S^{(t)}_2$ for some $t' < t$, then define $S^{(t-1)}_1 \triangleq S^{(t-1)}_1 \cup \brc{t'}$ and $S^{(t-1)}_2\triangleq S^{(t)}_2 \backslash \brc{(t,t')}$. We collect some basic observations about these two set sequences:
    
    \begin{observation}\label{obs:singleton}
        For every $i\in S^{(T)}_1$, we have that $i\in S^{(i)}_1$.
    \end{observation}
    
    \begin{observation}\label{obs:pair}
        For every $(i,i')\in S^{(T)}_2$, if $i\le i'$ then $i\in S^{(i)}_1$ while $i'\not\in S^{(i')}_1$.
    \end{observation}
    
    The reason for defining these set sequences is that we can extract $\wt{\rho}_{v_T}$ from the product on the right-hand side of \eqref{eq:prodRs} and apply \eqref{E:1tracebound1} (resp. \eqref{E:2tracebound1}) if $T\in S^{(T)}_1$ (resp. $(T,t')\in S^{(T)}_2$ for some $t' < T$) to obtain \begin{equation}
        \label{eq:induct_prodRs}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j = d^{\bone{T\in S^{(T)}_1}}\sum_{u: \,\text{depth}(u) = T - 1} (dd')^{T-1} W_u \prod_{i\in S^{(T-1)}_1} \Tr(\wt{\rho}_{v_i}) \cdot \prod_{(i,i') \in S^{(T-1)}_2} \Tr(\wt{\rho}_{v_i}\wt{\rho}_{v_{i'}}),
    \end{equation} where $W_u = w_{v_1}\cdots w_{v_{T-1}}$ if the path from root to $u$ in $\calT$ consists of $v_1,\ldots,v_{T-1} = u$.
    Proceeding inductively, we can express the right-hand side of \eqref{eq:induct_prodRs} as \begin{equation}
        d^{\sum^T_{t=1} \bone{t\in S^{(t)}_1}}.
    \end{equation} By Observations~\ref{obs:singleton} and \ref{obs:pair}, $\sum^T_{t=1}\bone{t\in S^{(t)}_1} = |S^{(T)}_1| + |S^{(T)}_2|$. Because every even cycle $C_m$ of $\tau^{-1}$ contributes $|C_m|/2$ pairs to $S^{(T)}_2$, and every odd cycle $C_m$ contributes $\floor{|C_m|/2}$ pairs to $S^{(T)}_2$ and one element to $S^{(T)}_1$, we conclude that
    \begin{align}
        \label{E:sboundhard2}
        \sum_{\ell\in\leaf(\calT)} (dd')^T W_{\ell} \prod_j R^{\ell}_j &= d^{\sum_{m=1}^{\#(\tau^{-1})} \left\lceil \frac{|C_m|}{2} \right\rceil} \nonumber \\
        &= d^{\frac{T}{2} - \sum_{m=1}^{\#(\tau^{-1})} \left\lfloor \frac{|C_m|}{2} \right\rfloor} \nonumber \\
        &\leq d^{\frac{T}{2} - \left\lfloor \frac{L(\tau^{-1})}{2} \right\rfloor}
    \end{align}
    as claimed.
\end{proof}
\textcolor{red}{[END OF PARTS WE NEED TO FIX]}
    
Putting all our previous bounds together, in particular Eq.~\eqref{E:Othirdterm1},~\eqref{E:OHolder2},~\eqref{E:Othirdterm1},~\eqref{E:Ocycledecomp1},~\eqref{E:Oproductwithsqrt1},~\eqref{E:multipleTs},~\eqref{E:sboundhard1}, we arrive at
\begin{equation}
\sum_{\ell \, \in \, \text{leaf}(\mathcal{T})} \sum_{\mathfrak{n} \not = \mathfrak{e}, \,\mathfrak{m}}|p_{\sigma, \tau}^{\mathcal{S}}(\ell)| \leq d^{T} \sum_{\mathfrak{m}} |\text{Wg}^{\text{Sp}}(\sigma_{\mathfrak{m}}^{-1}, d/2)| \sum_{\mathfrak{n} \not = \mathfrak{e}} d^{- \left\lfloor \frac{L^{\text{Sp}}(\mathfrak{n})}{4} \right\rfloor} \,.
\end{equation}
The first sum on the right-hand side is bounded by $d^T \sum_{\mathfrak{m}} |\text{Wg}^{\text{Sp}}(\sigma_{\mathfrak{m}}^{-1}, d/2)| \leq 1 + \mathcal{O}\!\left( \frac{T^2}{d}\right)$.  Considering the second sum on the right-hand side, let $N^{\text{Sp}}(T,\ell)$ be the number of permutations in $S_T$ where the length of the longest $M_{2T}$-cycle is $2\ell$.  Since $N^{\text{Sp}}(T,\ell) = N^O(T,\ell)$,  the second sum can be written as
\begin{equation}
\label{E:sumNTell}
\sum_{\ell = 2}^T N^{\text{Sp}}(T,\ell) \, d^{- \left\lfloor \frac{\ell}{2} \right\rfloor} \leq \frac{T^3}{d} + \frac{T^2}{d} + \mathcal{O}\!\left(\frac{T^5}{d^2}\right)\,.
\end{equation}
%we observe that the number of permutations of $T$ items with $L$ disjoint cycles (including counting cycles of unit length) is given by the unsigned Stirling numbers of the first kind ${ T\brack L}$.  As such we can write
%\begin{equation}
%\label{E:1stirling1}
%\sum_{\tau \not = \mathds{1}} d^{\#(\tau^{-1})/2}  = \sum_{L=0}^{T-1} { T\brack L}  d^{L/2} 
%\end{equation}
%where we only sum up to $T-1$ since $L = T$ corresponds to $\tau^{-1} = \mathds{1}$ which is omitted from the sum.  Unsigned Stirling numbers of the first kind enjoy the identity $\sum_{L=0}^T { T\brack L} \, x^L = x (x+1) \cdots (x + T - 1)$ and so~\eqref{E:1stirling1} is equivalent to
%\begin{align}
%d^{1/2} \left(d^{1/2}  + 1\right) \cdots \left(d^{1/2}  + T-1 \right) - d^{T/2} &\le d^{T/2}\left(\exp\left(\frac{T(T-1)}{d^{1/2}}\right) - 1\right).
%\end{align}
Now if $T \le o(d^{1/3})$, then this quantity is $o(1)$ for some absolute constant $c > 0$. Altogether, we find
\begin{equation}
\frac{1}{2}\sum_{\ell\,\in\,\text{leaf}(\mathcal{T})} \sum_{\mathfrak{n}\not = \mathfrak{e}, \,\mathfrak{m}}|p_{\mathfrak{m}, \mathfrak{n}}^{\mathcal{S}}(\ell)| \leq o\!\left(1\right)\,.
\end{equation}
% \\ \\
% \indent In totality, for $T \leq \frac{\sqrt{d}}{4}$ we find
% \begin{equation}
% \frac{1}{2}\sum_s |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)]| \leq o\!\left(1\right)
% \end{equation}
% which is the claimed result.

\end{proof}

==> scratch.tex <==
We begin by writing
\begin{equation}
\frac{1}{2}\sum_{\ell \,\in\,\text{leaf}(\mathcal{T})} |p^{\mathcal{D}}(\ell) - \mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)]| = \sum_{\ell \,\in\,\text{leaf}_{\geq}\!(\mathcal{T})} \!\!\left(\mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)] - p^{\mathcal{D}}(\ell)\right)
\end{equation}
where $\text{leaf}_{\geq}(\mathcal{T})$ denotes the leaves of $\mathcal{T}$ such that $\mathbb{E}_{\text{Haar}}[p^{\mathcal{U}}(\ell)] \geq p^{\mathcal{D}}(\ell)$.  We then decompose the right-hand side as
\begin{align}
\label{E:firstineq1}
\sum_{\ell \,\in\,\text{leaf}_{\geq}\!(\mathcal{T})}\!\!\left(p_{\mathds{1},\mathds{1}}(\ell) - p^{\mathcal{D}}(\ell)\right) + \sum_{\ell \,\in\,\text{leaf}_{\geq}\!(\mathcal{T})} \sum_{\sigma \not = \mathds{1}} \, p_{\sigma, \mathds{1}}(\ell) +  \sum_{\ell \,\in\,\text{leaf}_{\geq}\!(\mathcal{T})} \sum_{\tau \not = \mathds{1}, \,\sigma}p_{\sigma, \tau}(\ell) \,.
\end{align}
We will bound each term in turn.  Further applying Cauchy-Schwarz to the first term we find that it is less than or equal to
\begin{align}
\label{E:11bound}
    \includegraphics[scale=.32, valign = c]{11bound.png}
\end{align}
Since by Corollary~\ref{cor:WgU1bd} we have $|\text{Wg}^U(\mathds{1},d) - \frac{1}{d^k}| \leq \mathcal{O}(k^{7/2}/d^{k+2})$ for $k < \left(\frac{d}{\sqrt{6}}\right)^{4/7}$, it follows that
\begin{equation}
p_{\mathds{1},\mathds{1}}(\ell) - p^{\mathcal{D}}(\ell) \leq \mathcal{O}\!\left(\frac{k^{7/2}}{D^2}\right)\,.
\end{equation}
